NLO QCD and electroweak corrections to W+\gamma\ production with leptonic W-boson decays

We present a calculation of the next-to-leading-order electroweak corrections to W+\gamma\ production, including the leptonic decay of the W boson and taking into account all off-shell effects of the W boson, where the finite width of the W boson is implemented using the complex-mass scheme. Corrections induced by incoming photons are fully included and find particular emphasis in the discussion of phenomenological predictions for the LHC. The corresponding next-to-leading-order QCD corrections are reproduced as well. In order to separate hard photons from jets, a quark-to-photon fragmentation function a la Glover and Morgan is employed. Our results are implemented into Monte Carlo programs allowing for the evaluation of arbitrary differential cross sections. We present integrated cross sections for the LHC at 7TeV, 8TeV, and 14TeV as well as differential distributions at 14TeV for bare muons and dressed leptons. Finally, we discuss the impact of anomalous WW\gamma\ couplings.

==> plots/feynman_diagrams/real_qph/qph_real01.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(10.,5.5)(0.,){Straight}{1}
\FALabel(2.69219,13.7012)[bl]{$u$}
\FAProp(0.,5.)(10.,14.5)(0.,){Sine}{0}
\FALabel(2.69219,6.29875)[tl]{$\gamma$}
\FAProp(20.,18.)(15.5,15.)(0.,){Straight}{1}
\FALabel(17.3702,17.3097)[br]{$l^+$}
\FAProp(20.,12.)(15.5,15.)(0.,){Straight}{-1}
\FALabel(18.1298,14.3097)[bl]{$\nu_l$}
\FAProp(20.,8.)(10.,14.5)(0.,){Sine}{0}
\FALabel(16.8438,8.77039)[tr]{$\gamma$}
\FAProp(20.,2.)(10.,5.5)(0.,){Straight}{-1}
\FALabel(14.488,2.76702)[t]{$d$}
\FAProp(10.,5.5)(10.,14.5)(0.,){Sine}{-1}
\FALabel(11.07,10.)[l]{$W$}
\FAProp(15.5,15.)(10.,14.5)(0.,){Sine}{1}
\FALabel(12.6097,15.8136)[b]{$W$}
\FAVert(10.,5.5){0}
\FAVert(15.5,15.){0}
\FAVert(10.,14.5){0}

\end{feynartspicture}



==> plots/feynman_diagrams/real_qph/qph_real02.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(4.,10.)(0.,){Straight}{1}
\FALabel(1.26965,12.0117)[tr]{$u$}
\FAProp(0.,5.)(4.,10.)(0.,){Sine}{0}
\FALabel(2.73035,7.01172)[tl]{$\gamma$}
\FAProp(20.,18.)(14.,15.)(0.,){Straight}{1}
\FALabel(16.7868,17.4064)[br]{$l^+$}
\FAProp(20.,12.)(14.,15.)(0.,){Straight}{-1}
\FALabel(16.7868,12.5936)[tr]{$\nu_l$}
\FAProp(20.,8.)(14.,5.)(0.,){Sine}{0}
\FALabel(16.7868,7.40636)[br]{$\gamma$}
\FAProp(20.,2.)(14.,5.)(0.,){Straight}{-1}
\FALabel(16.7868,2.59364)[tr]{$d$}
\FAProp(4.,10.)(10.,10.)(0.,){Straight}{1}
\FALabel(7.,11.07)[b]{$u$}
\FAProp(14.,15.)(10.,10.)(0.,){Sine}{1}
\FALabel(11.2697,12.9883)[br]{$W$}
\FAProp(14.,5.)(10.,10.)(0.,){Straight}{-1}
\FALabel(11.2697,7.01172)[tr]{$d$}
\FAVert(4.,10.){0}
\FAVert(14.,15.){0}
\FAVert(14.,5.){0}
\FAVert(10.,10.){0}

\end{feynartspicture}



==> plots/feynman_diagrams/real_qph/qph_real03.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(3.5,10.)(0.,){Straight}{1}
\FALabel(2.53981,12.9089)[bl]{$u$}
\FAProp(0.,5.)(3.5,10.)(0.,){Sine}{0}
\FALabel(0.960191,7.90887)[br]{$\gamma$}
\FAProp(20.,18.)(15.5,15.)(0.,){Straight}{1}
\FALabel(17.3702,17.3097)[br]{$l^+$}
\FAProp(20.,12.)(15.5,15.)(0.,){Straight}{-1}
\FALabel(17.3702,12.6903)[tr]{$\nu_l$}
\FAProp(20.,8.)(9.,7.)(0.,){Sine}{0}
\FALabel(11.0226,5.73103)[t]{$\gamma$}
\FAProp(20.,2.)(10.5,13.)(0.,){Straight}{-1}
\FALabel(17.2908,3.3166)[tr]{$d$}
\FAProp(3.5,10.)(9.,7.)(0.,){Straight}{1}
\FALabel(5.98778,7.61926)[tr]{$u$}
\FAProp(15.5,15.)(10.5,13.)(0.,){Sine}{1}
\FALabel(12.4243,14.9591)[b]{$W$}
\FAProp(9.,7.)(10.5,13.)(0.,){Straight}{1}
\FALabel(8.72628,10.3759)[r]{$u$}
\FAVert(3.5,10.){0}
\FAVert(15.5,15.){0}
\FAVert(9.,7.){0}
\FAVert(10.5,13.){0}

\end{feynartspicture}



==> plots/feynman_diagrams/real_qph/qph_real04.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(4.,10.)(0.,){Straight}{1}
\FALabel(2.73035,12.9883)[bl]{$u$}
\FAProp(0.,5.)(4.,10.)(0.,){Sine}{0}
\FALabel(1.26965,7.98828)[br]{$\gamma$}
\FAProp(20.,18.)(15.5,15.)(0.,){Straight}{1}
\FALabel(17.3702,17.3097)[br]{$l^+$}
\FAProp(20.,12.)(15.5,15.)(0.,){Straight}{-1}
\FALabel(17.3702,12.6903)[tr]{$\nu_l$}
\FAProp(20.,8.)(11.5,12.5)(0.,){Sine}{0}
\FALabel(15.5048,9.36013)[tr]{$\gamma$}
\FAProp(20.,2.)(8.,9.)(0.,){Straight}{-1}
\FALabel(13.699,4.64114)[tr]{$d$}
\FAProp(4.,10.)(8.,9.)(0.,){Straight}{1}
\FALabel(5.62407,8.47628)[t]{$u$}
\FAProp(15.5,15.)(11.5,12.5)(0.,){Sine}{1}
\FALabel(13.1585,14.5844)[br]{$W$}
\FAProp(11.5,12.5)(8.,9.)(0.,){Sine}{1}
\FALabel(9.13398,11.366)[br]{$W$}
\FAVert(4.,10.){0}
\FAVert(15.5,15.){0}
\FAVert(11.5,12.5){0}
\FAVert(8.,9.){0}

\end{feynartspicture}



==> plots/feynman_diagrams/real_qph/qph_real05.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(4.5,10.)(0.,){Straight}{1}
\FALabel(1.57789,11.9431)[tr]{$u$}
\FAProp(0.,5.)(4.5,10.)(0.,){Sine}{0}
\FALabel(2.92211,6.9431)[tl]{$\gamma$}
\FAProp(20.,18.)(14.5,16.)(0.,){Straight}{1}
\FALabel(16.7203,17.9767)[b]{$l^+$}
\FAProp(20.,12.)(11.5,13.)(0.,){Straight}{-1}
\FALabel(13.9708,11.7317)[t]{$\nu_l$}
\FAProp(20.,8.)(14.5,16.)(0.,){Sine}{0}
\FALabel(18.274,8.83837)[tr]{$\gamma$}
\FAProp(20.,2.)(8.5,10.)(0.,){Straight}{-1}
\FALabel(13.8449,5.2076)[tr]{$d$}
\FAProp(4.5,10.)(8.5,10.)(0.,){Straight}{1}
\FALabel(6.5,8.93)[t]{$u$}
\FAProp(14.5,16.)(11.5,13.)(0.,){Straight}{1}
\FALabel(12.384,15.116)[br]{$l^+$}
\FAProp(11.5,13.)(8.5,10.)(0.,){Sine}{1}
\FALabel(9.38398,12.116)[br]{$W$}
\FAVert(4.5,10.){0}
\FAVert(14.5,16.){0}
\FAVert(11.5,13.){0}
\FAVert(8.5,10.){0}

\end{feynartspicture}



==> plots/feynman_diagrams/real_qph/qph_real06.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(8.,15.5)(0.,){Straight}{1}
\FALabel(3.90331,16.317)[b]{$u$}
\FAProp(0.,5.)(8.,4.5)(0.,){Sine}{0}
\FALabel(3.90331,3.68302)[t]{$\gamma$}
\FAProp(20.,18.)(8.,4.5)(0.,){Straight}{1}
\FALabel(17.2931,16.6861)[br]{$l^+$}
\FAProp(20.,12.)(8.,8.)(0.,){Straight}{-1}
\FALabel(17.9209,12.7572)[b]{$\nu_l$}
\FAProp(20.,8.)(8.,15.5)(0.,){Sine}{0}
\FALabel(11.1525,15.232)[bl]{$\gamma$}
\FAProp(20.,2.)(8.,12.)(0.,){Straight}{-1}
\FALabel(15.32,4.28794)[tr]{$d$}
\FAProp(8.,15.5)(8.,12.)(0.,){Straight}{1}
\FALabel(6.93,13.75)[r]{$u$}
\FAProp(8.,4.5)(8.,8.)(0.,){Straight}{1}
\FALabel(6.93,6.25)[r]{$l^+$}
\FAProp(8.,8.)(8.,12.)(0.,){Sine}{1}
\FALabel(6.93,10.)[r]{$W$}
\FAVert(8.,15.5){0}
\FAVert(8.,4.5){0}
\FAVert(8.,8.){0}
\FAVert(8.,12.){0}

\end{feynartspicture}



==> plots/feynman_diagrams/real_qph/qph_real07.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(10.,4.5)(0.,){Straight}{1}
\FALabel(3.20103,13.1924)[bl]{$u$}
\FAProp(0.,5.)(10.,15.5)(0.,){Sine}{0}
\FALabel(3.20103,6.80759)[tl]{$\gamma$}
\FAProp(20.,18.)(10.,15.5)(0.,){Straight}{1}
\FALabel(14.6241,17.7737)[b]{$l^+$}
\FAProp(20.,12.)(10.,8.)(0.,){Straight}{-1}
\FALabel(17.9072,12.7521)[b]{$\nu_l$}
\FAProp(20.,8.)(10.,12.)(0.,){Sine}{0}
\FALabel(17.9072,7.24788)[t]{$\gamma$}
\FAProp(20.,2.)(10.,4.5)(0.,){Straight}{-1}
\FALabel(14.6241,2.22628)[t]{$d$}
\FAProp(10.,4.5)(10.,8.)(0.,){Sine}{-1}
\FALabel(11.07,6.25)[l]{$W$}
\FAProp(10.,15.5)(10.,12.)(0.,){Straight}{1}
\FALabel(11.07,13.75)[l]{$l^+$}
\FAProp(10.,8.)(10.,12.)(0.,){Straight}{-1}
\FALabel(8.93,10.)[r]{$l^+$}
\FAVert(10.,4.5){0}
\FAVert(10.,15.5){0}
\FAVert(10.,8.){0}
\FAVert(10.,12.){0}

\end{feynartspicture}



==> plots/feynman_diagrams/real_qph/qph_real08.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(10.,4.5)(0.,){Straight}{1}
\FALabel(3.20103,13.1924)[bl]{$u$}
\FAProp(0.,5.)(10.,15.5)(0.,){Sine}{0}
\FALabel(3.20103,6.80759)[tl]{$\gamma$}
\FAProp(20.,18.)(10.,15.5)(0.,){Straight}{1}
\FALabel(14.6241,17.7737)[b]{$l^+$}
\FAProp(20.,12.)(10.,12.)(0.,){Straight}{-1}
\FALabel(16.,12.77)[b]{$\nu_l$}
\FAProp(20.,8.)(10.,8.)(0.,){Sine}{0}
\FALabel(16.,8.77)[b]{$\gamma$}
\FAProp(20.,2.)(10.,4.5)(0.,){Straight}{-1}
\FALabel(14.6241,2.22628)[t]{$d$}
\FAProp(10.,4.5)(10.,8.)(0.,){Sine}{-1}
\FALabel(11.07,6.25)[l]{$W$}
\FAProp(10.,15.5)(10.,12.)(0.,){Straight}{1}
\FALabel(11.07,13.75)[l]{$l^+$}
\FAProp(10.,12.)(10.,8.)(0.,){Sine}{1}
\FALabel(11.07,10.)[l]{$W$}
\FAVert(10.,4.5){0}
\FAVert(10.,15.5){0}
\FAVert(10.,12.){0}
\FAVert(10.,8.){0}

\end{feynartspicture}



==> plots/feynman_diagrams/real_qph/qph_real09.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(10.,5.5)(0.,){Straight}{1}
\FALabel(3.19219,13.2012)[bl]{$u$}
\FAProp(0.,5.)(10.,14.5)(0.,){Sine}{0}
\FALabel(3.19219,6.79875)[tl]{$\gamma$}
\FAProp(20.,18.)(10.,14.5)(0.,){Straight}{1}
\FALabel(14.488,17.233)[b]{$l^+$}
\FAProp(20.,12.)(10.,10.)(0.,){Straight}{-1}
\FALabel(15.951,12.2651)[b]{$\nu_l$}
\FAProp(20.,8.)(15.5,5.)(0.,){Sine}{0}
\FALabel(17.3702,7.30968)[br]{$\gamma$}
\FAProp(20.,2.)(15.5,5.)(0.,){Straight}{-1}
\FALabel(18.1298,4.30968)[bl]{$d$}
\FAProp(10.,5.5)(10.,10.)(0.,){Sine}{-1}
\FALabel(11.07,7.75)[l]{$W$}
\FAProp(10.,5.5)(15.5,5.)(0.,){Straight}{1}
\FALabel(12.6097,4.18637)[t]{$d$}
\FAProp(10.,14.5)(10.,10.)(0.,){Straight}{1}
\FALabel(11.07,12.25)[l]{$l^+$}
\FAVert(10.,5.5){0}
\FAVert(10.,14.5){0}
\FAVert(10.,10.){0}
\FAVert(15.5,5.){0}

\end{feynartspicture}



==> plots/feynman_diagrams/real_qph/qph_real10.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(8.,14.5)(0.,){Straight}{1}
\FALabel(4.09669,15.817)[b]{$u$}
\FAProp(0.,5.)(8.,5.5)(0.,){Sine}{0}
\FALabel(4.09669,4.18302)[t]{$\gamma$}
\FAProp(20.,18.)(15.5,15.)(0.,){Straight}{1}
\FALabel(17.3702,17.3097)[br]{$l^+$}
\FAProp(20.,12.)(15.5,15.)(0.,){Straight}{-1}
\FALabel(18.1298,14.3097)[bl]{$\nu_l$}
\FAProp(20.,8.)(8.,14.5)(0.,){Sine}{0}
\FALabel(16.2504,8.85404)[tr]{$\gamma$}
\FAProp(20.,2.)(8.,5.5)(0.,){Straight}{-1}
\FALabel(13.566,2.742)[t]{$d$}
\FAProp(8.,14.5)(8.,10.)(0.,){Straight}{1}
\FALabel(6.93,12.25)[r]{$u$}
\FAProp(8.,5.5)(8.,10.)(0.,){Straight}{-1}
\FALabel(6.93,7.75)[r]{$d$}
\FAProp(15.5,15.)(8.,10.)(0.,){Sine}{1}
\FALabel(13.2061,14.5881)[br]{$W$}
\FAVert(8.,14.5){0}
\FAVert(8.,5.5){0}
\FAVert(15.5,15.){0}
\FAVert(8.,10.){0}

\end{feynartspicture}



==> plots/feynman_diagrams/real_qph/qph_real11.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(8.,14.5)(0.,){Straight}{1}
\FALabel(4.09669,15.817)[b]{$u$}
\FAProp(0.,5.)(8.,5.5)(0.,){Sine}{0}
\FALabel(4.09669,4.18302)[t]{$\gamma$}
\FAProp(20.,18.)(16.5,15.)(0.,){Straight}{1}
\FALabel(17.7213,17.1968)[br]{$l^+$}
\FAProp(20.,12.)(16.5,15.)(0.,){Straight}{-1}
\FALabel(18.7787,14.1968)[bl]{$\nu_l$}
\FAProp(20.,8.)(8.,14.5)(0.,){Sine}{0}
\FALabel(11.1391,14.2398)[bl]{$\gamma$}
\FAProp(20.,2.)(13.,6.)(0.,){Straight}{-1}
\FALabel(16.211,3.13422)[tr]{$d$}
\FAProp(8.,14.5)(8.,5.5)(0.,){Straight}{1}
\FALabel(6.93,10.)[r]{$u$}
\FAProp(8.,5.5)(13.,6.)(0.,){Straight}{1}
\FALabel(10.6542,4.68769)[t]{$u$}
\FAProp(16.5,15.)(13.,6.)(0.,){Sine}{1}
\FALabel(14.753,7.40939)[l]{$W$}
\FAVert(8.,14.5){0}
\FAVert(8.,5.5){0}
\FAVert(16.5,15.){0}
\FAVert(13.,6.){0}

\end{feynartspicture}



==> plots/feynman_diagrams/real_qph/qph_real12.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(8.,14.5)(0.,){Straight}{1}
\FALabel(4.09669,15.817)[b]{$u$}
\FAProp(0.,5.)(8.,5.5)(0.,){Sine}{0}
\FALabel(4.09669,4.18302)[t]{$\gamma$}
\FAProp(20.,18.)(16.5,15.)(0.,){Straight}{1}
\FALabel(17.7213,17.1968)[br]{$l^+$}
\FAProp(20.,12.)(16.5,15.)(0.,){Straight}{-1}
\FALabel(18.7787,14.1968)[bl]{$\nu_l$}
\FAProp(20.,8.)(8.,14.5)(0.,){Sine}{0}
\FALabel(17.1125,8.47023)[tr]{$\gamma$}
\FAProp(20.,2.)(8.,10.)(0.,){Straight}{-1}
\FALabel(15.8413,3.27199)[tr]{$d$}
\FAProp(8.,14.5)(8.,10.)(0.,){Straight}{1}
\FALabel(6.93,12.25)[r]{$u$}
\FAProp(8.,5.5)(16.5,15.)(0.,){Sine}{-1}
\FALabel(14.0417,13.4553)[br]{$W$}
\FAProp(8.,5.5)(8.,10.)(0.,){Sine}{1}
\FALabel(6.93,7.75)[r]{$W$}
\FAVert(8.,14.5){0}
\FAVert(8.,5.5){0}
\FAVert(16.5,15.){0}
\FAVert(8.,10.){0}

\end{feynartspicture}



==> plots/feynman_diagrams/real_qph/qph_real13.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(10.,5.5)(0.,){Straight}{1}
\FALabel(3.19219,13.2012)[bl]{$u$}
\FAProp(0.,5.)(10.,14.5)(0.,){Sine}{0}
\FALabel(3.19219,6.79875)[tl]{$\gamma$}
\FAProp(20.,18.)(17.,15.)(0.,){Straight}{1}
\FALabel(17.884,17.116)[br]{$l^+$}
\FAProp(20.,12.)(17.,15.)(0.,){Straight}{-1}
\FALabel(19.116,14.116)[bl]{$\nu_l$}
\FAProp(20.,8.)(13.5,14.)(0.,){Sine}{0}
\FALabel(16.1787,10.3411)[tr]{$\gamma$}
\FAProp(20.,2.)(10.,5.5)(0.,){Straight}{-1}
\FALabel(14.488,2.76702)[t]{$d$}
\FAProp(10.,5.5)(10.,14.5)(0.,){Sine}{-1}
\FALabel(11.27,8.5)[l]{$W$}
\FAProp(10.,14.5)(13.5,14.)(0.,){ScalarDash}{-1}
\FALabel(11.9692,15.3044)[b]{$G$}
\FAProp(17.,15.)(13.5,14.)(0.,){Sine}{1}
\FALabel(14.8242,15.5104)[b]{$W$}
\FAVert(10.,5.5){0}
\FAVert(10.,14.5){0}
\FAVert(17.,15.){0}
\FAVert(13.5,14.){0}

\end{feynartspicture}



==> plots/feynman_diagrams/real_qph/qph_real14.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(10.,5.5)(0.,){Straight}{1}
\FALabel(3.19219,13.2012)[bl]{$u$}
\FAProp(0.,5.)(10.,14.5)(0.,){Sine}{0}
\FALabel(3.19219,6.79875)[tl]{$\gamma$}
\FAProp(20.,18.)(17.,15.)(0.,){Straight}{1}
\FALabel(17.884,17.116)[br]{$l^+$}
\FAProp(20.,12.)(17.,15.)(0.,){Straight}{-1}
\FALabel(19.116,14.116)[bl]{$\nu_l$}
\FAProp(20.,8.)(13.5,14.)(0.,){Sine}{0}
\FALabel(16.1787,10.3411)[tr]{$\gamma$}
\FAProp(20.,2.)(10.,5.5)(0.,){Straight}{-1}
\FALabel(14.488,2.76702)[t]{$d$}
\FAProp(10.,5.5)(10.,14.5)(0.,){Sine}{-1}
\FALabel(11.27,8.5)[l]{$W$}
\FAProp(10.,14.5)(13.5,14.)(0.,){Sine}{-1}
\FALabel(11.9692,15.3044)[b]{$W$}
\FAProp(17.,15.)(13.5,14.)(0.,){Sine}{1}
\FALabel(14.8242,15.5104)[b]{$W$}
\FAVert(10.,5.5){0}
\FAVert(10.,14.5){0}
\FAVert(17.,15.){0}
\FAVert(13.5,14.){0}

\end{feynartspicture}



==> plots/feynman_diagrams/real_qph/qph_real15.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(10.,5.5)(0.,){Straight}{1}
\FALabel(3.19219,13.2012)[bl]{$u$}
\FAProp(0.,5.)(10.,14.5)(0.,){Sine}{0}
\FALabel(3.19219,6.79875)[tl]{$\gamma$}
\FAProp(20.,18.)(15.5,15.)(0.,){Straight}{1}
\FALabel(18.1298,15.6903)[tl]{$l^+$}
\FAProp(20.,12.)(15.5,15.)(0.,){Straight}{-1}
\FALabel(17.3702,12.6903)[tr]{$\nu_l$}
\FAProp(20.,8.)(10.,10.)(0.,){Sine}{0}
\FALabel(15.951,7.73485)[t]{$\gamma$}
\FAProp(20.,2.)(10.,5.5)(0.,){Straight}{-1}
\FALabel(14.488,2.76702)[t]{$d$}
\FAProp(10.,5.5)(10.,10.)(0.,){Sine}{-1}
\FALabel(11.07,7.75)[l]{$W$}
\FAProp(10.,14.5)(15.5,15.)(0.,){Sine}{-1}
\FALabel(12.6097,15.8136)[b]{$W$}
\FAProp(10.,14.5)(10.,10.)(0.,){ScalarDash}{1}
\FALabel(11.07,12.25)[l]{$G$}
\FAVert(10.,5.5){0}
\FAVert(10.,14.5){0}
\FAVert(15.5,15.){0}
\FAVert(10.,10.){0}

\end{feynartspicture}



==> plots/feynman_diagrams/real_qph/qph_real16.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(10.,5.5)(0.,){Straight}{1}
\FALabel(3.19219,13.2012)[bl]{$u$}
\FAProp(0.,5.)(10.,14.5)(0.,){Sine}{0}
\FALabel(3.19219,6.79875)[tl]{$\gamma$}
\FAProp(20.,18.)(15.5,15.)(0.,){Straight}{1}
\FALabel(18.1298,15.6903)[tl]{$l^+$}
\FAProp(20.,12.)(15.5,15.)(0.,){Straight}{-1}
\FALabel(17.3702,12.6903)[tr]{$\nu_l$}
\FAProp(20.,8.)(10.,10.)(0.,){Sine}{0}
\FALabel(15.951,7.73485)[t]{$\gamma$}
\FAProp(20.,2.)(10.,5.5)(0.,){Straight}{-1}
\FALabel(14.488,2.76702)[t]{$d$}
\FAProp(10.,5.5)(10.,10.)(0.,){Sine}{-1}
\FALabel(11.07,7.75)[l]{$W$}
\FAProp(10.,14.5)(15.5,15.)(0.,){Sine}{-1}
\FALabel(12.6097,15.8136)[b]{$W$}
\FAProp(10.,14.5)(10.,10.)(0.,){Sine}{1}
\FALabel(11.07,12.25)[l]{$W$}
\FAVert(10.,5.5){0}
\FAVert(10.,14.5){0}
\FAVert(15.5,15.){0}
\FAVert(10.,10.){0}

\end{feynartspicture}



==> plots/feynman_diagrams/real_qph/qph_real17.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(8.,14.5)(0.,){Straight}{1}
\FALabel(4.09669,15.817)[b]{$u$}
\FAProp(0.,5.)(8.,5.5)(0.,){Sine}{0}
\FALabel(4.09669,4.18302)[t]{$\gamma$}
\FAProp(20.,18.)(16.,15.)(0.,){Straight}{1}
\FALabel(17.55,17.26)[br]{$l^+$}
\FAProp(20.,12.)(16.,15.)(0.,){Straight}{-1}
\FALabel(18.45,14.26)[bl]{$\nu_l$}
\FAProp(20.,8.)(12.,14.)(0.,){Sine}{0}
\FALabel(15.55,10.24)[tr]{$\gamma$}
\FAProp(20.,2.)(8.,5.5)(0.,){Straight}{-1}
\FALabel(13.566,2.742)[t]{$d$}
\FAProp(8.,14.5)(8.,5.5)(0.,){Straight}{1}
\FALabel(6.93,10.)[r]{$d$}
\FAProp(8.,14.5)(12.,14.)(0.,){Sine}{-1}
\FALabel(10.1923,15.308)[b]{$W$}
\FAProp(16.,15.)(12.,14.)(0.,){Sine}{1}
\FALabel(13.6241,15.5237)[b]{$W$}
\FAVert(8.,14.5){0}
\FAVert(8.,5.5){0}
\FAVert(16.,15.){0}
\FAVert(12.,14.){0}

\end{feynartspicture}



==> plots/feynman_diagrams/real_qph/qph_real18.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(8.,14.5)(0.,){Straight}{1}
\FALabel(4.09669,15.817)[b]{$u$}
\FAProp(0.,5.)(8.,5.5)(0.,){Sine}{0}
\FALabel(4.09669,4.18302)[t]{$\gamma$}
\FAProp(20.,18.)(14.5,15.)(0.,){Straight}{1}
\FALabel(16.9878,17.3807)[br]{$l^+$}
\FAProp(20.,12.)(14.5,15.)(0.,){Straight}{-1}
\FALabel(16.9878,12.6193)[tr]{$\nu_l$}
\FAProp(20.,8.)(8.,10.)(0.,){Sine}{0}
\FALabel(13.7452,7.95109)[t]{$\gamma$}
\FAProp(20.,2.)(8.,5.5)(0.,){Straight}{-1}
\FALabel(13.566,2.742)[t]{$d$}
\FAProp(8.,14.5)(14.5,15.)(0.,){Sine}{-1}
\FALabel(11.1311,15.8154)[b]{$W$}
\FAProp(8.,14.5)(8.,10.)(0.,){Straight}{1}
\FALabel(6.93,12.25)[r]{$d$}
\FAProp(8.,5.5)(8.,10.)(0.,){Straight}{-1}
\FALabel(6.93,7.75)[r]{$d$}
\FAVert(8.,14.5){0}
\FAVert(8.,5.5){0}
\FAVert(14.5,15.){0}
\FAVert(8.,10.){0}

\end{feynartspicture}



==> plots/feynman_diagrams/real_qph/qph_real19.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(8.,14.5)(0.,){Straight}{1}
\FALabel(4.09669,15.817)[b]{$u$}
\FAProp(0.,5.)(8.,5.5)(0.,){Sine}{0}
\FALabel(4.09669,4.18302)[t]{$\gamma$}
\FAProp(20.,18.)(14.,15.)(0.,){Straight}{1}
\FALabel(16.7868,17.4064)[br]{$l^+$}
\FAProp(20.,12.)(14.,15.)(0.,){Straight}{-1}
\FALabel(16.7868,12.5936)[tr]{$\nu_l$}
\FAProp(20.,8.)(14.,5.)(0.,){Sine}{0}
\FALabel(16.7868,7.40636)[br]{$\gamma$}
\FAProp(20.,2.)(14.,5.)(0.,){Straight}{-1}
\FALabel(16.7868,2.59364)[tr]{$d$}
\FAProp(8.,14.5)(8.,5.5)(0.,){Straight}{1}
\FALabel(6.93,10.)[r]{$d$}
\FAProp(8.,14.5)(14.,15.)(0.,){Sine}{-1}
\FALabel(10.8713,15.8146)[b]{$W$}
\FAProp(8.,5.5)(14.,5.)(0.,){Straight}{1}
\FALabel(10.8713,4.18535)[t]{$d$}
\FAVert(8.,14.5){0}
\FAVert(8.,5.5){0}
\FAVert(14.,15.){0}
\FAVert(14.,5.){0}

\end{feynartspicture}



==> plots/feynman_diagrams/real_qph/qph_real20.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(10.,5.5)(0.,){Straight}{1}
\FALabel(4.19219,13.2012)[bl]{$u$}
\FAProp(0.,5.)(10.,14.5)(0.,){Sine}{0}
\FALabel(4.19219,6.79875)[tl]{$\gamma$}
\FAProp(20.,18.)(15.,15.)(0.,){Straight}{1}
\FALabel(17.1825,17.3491)[br]{$l^+$}
\FAProp(20.,12.)(15.,15.)(0.,){Straight}{-1}
\FALabel(17.1825,12.6509)[tr]{$\nu_l$}
\FAProp(20.,8.)(15.,5.)(0.,){Sine}{0}
\FALabel(17.1825,7.34911)[br]{$\gamma$}
\FAProp(20.,2.)(15.,5.)(0.,){Straight}{-1}
\FALabel(17.1825,2.65089)[tr]{$d$}
\FAProp(10.,5.5)(10.,14.5)(0.,){Sine}{-1}
\FALabel(11.07,10.)[l]{$W$}
\FAProp(10.,5.5)(15.,5.)(0.,){Straight}{1}
\FALabel(12.3458,4.18769)[t]{$d$}
\FAProp(10.,14.5)(15.,15.)(0.,){Sine}{-1}
\FALabel(12.3458,15.8123)[b]{$W$}
\FAVert(10.,5.5){0}
\FAVert(10.,14.5){0}
\FAVert(15.,15.){0}
\FAVert(15.,5.){0}

\end{feynartspicture}



==> plots/feynman_diagrams/real_qph/qph_real21.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(8.,14.5)(0.,){Straight}{1}
\FALabel(4.09669,15.817)[b]{$u$}
\FAProp(0.,5.)(8.,5.5)(0.,){Sine}{0}
\FALabel(4.09669,4.18302)[t]{$\gamma$}
\FAProp(20.,18.)(15.5,13.)(0.,){Straight}{1}
\FALabel(17.0779,16.0569)[br]{$l^+$}
\FAProp(20.,12.)(12.,8.)(0.,){Straight}{-1}
\FALabel(18.8368,12.4879)[br]{$\nu_l$}
\FAProp(20.,8.)(15.5,13.)(0.,){Sine}{0}
\FALabel(18.8851,7.76435)[tr]{$\gamma$}
\FAProp(20.,2.)(8.,14.5)(0.,){Straight}{-1}
\FALabel(16.7997,3.80687)[tr]{$d$}
\FAProp(8.,14.5)(8.,5.5)(0.,){Sine}{-1}
\FALabel(6.93,10.)[r]{$W$}
\FAProp(8.,5.5)(12.,8.)(0.,){Sine}{-1}
\FALabel(10.3415,5.9156)[tl]{$W$}
\FAProp(15.5,13.)(12.,8.)(0.,){Straight}{1}
\FALabel(13.7752,12.6634)[br]{$l^+$}
\FAVert(8.,14.5){0}
\FAVert(8.,5.5){0}
\FAVert(15.5,13.){0}
\FAVert(12.,8.){0}

\end{feynartspicture}



==> plots/feynman_diagrams/real_qph/qph_real22.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(8.,14.5)(0.,){Straight}{1}
\FALabel(4.09669,15.817)[b]{$u$}
\FAProp(0.,5.)(8.,5.5)(0.,){Sine}{0}
\FALabel(4.09669,4.18302)[t]{$\gamma$}
\FAProp(20.,18.)(13.,7.)(0.,){Straight}{1}
\FALabel(17.7691,16.6542)[br]{$l^+$}
\FAProp(20.,12.)(8.,10.)(0.,){Straight}{-1}
\FALabel(18.0229,10.6047)[t]{$\nu_l$}
\FAProp(20.,8.)(13.,7.)(0.,){Sine}{0}
\FALabel(18.4137,6.88281)[t]{$\gamma$}
\FAProp(20.,2.)(8.,14.5)(0.,){Straight}{-1}
\FALabel(16.7997,3.80687)[tr]{$d$}
\FAProp(8.,14.5)(8.,10.)(0.,){Sine}{-1}
\FALabel(6.93,12.25)[r]{$W$}
\FAProp(8.,5.5)(13.,7.)(0.,){Straight}{-1}
\FALabel(10.5718,4.74054)[t]{$l^+$}
\FAProp(8.,5.5)(8.,10.)(0.,){Straight}{1}
\FALabel(6.93,7.75)[r]{$l^+$}
\FAVert(8.,14.5){0}
\FAVert(8.,5.5){0}
\FAVert(13.,7.){0}
\FAVert(8.,10.){0}

\end{feynartspicture}



==> plots/feynman_diagrams/real_qph/qph_real23.tex <==
\unitlength=1bp%

\begin{feynartspicture}(80,80)(1,1)

\FADiagram{}
\FAProp(0.,15.)(8.,14.5)(0.,){Straight}{1}
\FALabel(4.09669,15.817)[b]{$u$}
\FAProp(0.,5.)(8.,5.5)(0.,){Sine}{0}
\FALabel(4.09669,4.18302)[t]{$\gamma$}
\FAProp(20.,18.)(17.5,15.)(0.,){Straight}{1}
\FALabel(18.0393,17.0123)[br]{$l^+$}
\FAProp(20.,12.)(12.5,14.)(0.,){Straight}{-1}
\FALabel(13.4356,12.7384)[t]{$\nu_l$}
\FAProp(20.,8.)(17.5,15.)(0.,){Sine}{0}
\FALabel(18.2446,8.91592)[r]{$\gamma$}
\FAProp(20.,2.)(8.,5.5)(0.,){Straight}{-1}
\FALabel(13.566,2.742)[t]{$d$}
\FAProp(8.,14.5)(8.,5.5)(0.,){Straight}{1}
\FALabel(6.93,10.)[r]{$d$}
\FAProp(8.,14.5)(12.5,14.)(0.,){Sine}{-1}
\FALabel(10.4212,15.3105)[b]{$W$}
\FAProp(17.5,15.)(12.5,14.)(0.,){Straight}{1}
\FALabel(14.696,15.5399)[b]{$l^+$}
\FAVert(8.,14.5){0}
\FAVert(8.,5.5){0}
\FAVert(17.5,15.){0}
\FAVert(12.5,14.){0}

\end{feynartspicture}


